ARMA Processes with Discrete-Continuous Excitation: Compressibility Beyond Sparsity

R\'enyi Information Dimension (RID) plays a central role in quantifying the compressibility of random variables with singularities in their distribution, encompassing and extending beyond the class of sparse sources. The RID, from a high perspective, presents the average number of bits that is needed for coding the i.i.d. samples of a random variable with high precision. There are two main extensions of the RID for stochastic processes: information dimension rate (IDR) and block information dimension (BID). In addition, a more recent approach towards the compressibility of stochastic processes revolves around the concept of $\epsilon$-achievable compression rates, which treat a random process as the limiting point of finite-dimensional random vectors and apply the compressed sensing tools on these random variables. While there is limited knowledge about the interplay of the the BID, the IDR, and $\epsilon$-achievable compression rates, the value of IDR and BID themselves are known only for very specific types of processes, namely i.i.d. sequences (i.e., discrete-domain white noise) and moving-average (MA) processes. This paper investigates the IDR and BID of discrete-time Auto-Regressive Moving-Average (ARMA) processes in general, and their relations with $\epsilon$-achievable compression rates when the excitation noise has a discrete-continuous measure. To elaborate, this paper shows that the RID and $\epsilon$-achievable compression rates of this type of processes are equal to that of their excitation noise. In other words, the samples of such ARMA processes can be compressed as much as their sparse excitation noise, although the samples themselves are by no means sparse. The results of this paper can be used to evaluate the compressibility of various types of locally correlated data with finite- or infinite-memory as they are often modelled via ARMA processes.

==> tikz/3dPlot.tex <==
\pgfplotsset{compat=newest}
 
\usetikzlibrary{positioning}

\begin{tikzpicture}[scale=0.6,every node/.style={scale=2}][font=\sffamily]
\definecolor{mycolor1}{rgb}{0.00000,0.44706,0.74118}%
\definecolor{mycolor2}{rgb}{0.63529,0.07843,0.18431}%
\definecolor{mycolor3}{rgb}{0.00000,0.49804,0.00000}%
\definecolor{mycolor4}{rgb}{0.87059,0.49020,0.00000}%
\definecolor{mycolor5}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor6}{rgb}{0.74902,0.00000,0.74902}%

\begin{axis}[width=0.75*\textwidth,
                axis lines=left,
                xlabel=$X_1$,
                ylabel=$X_2$,
                zlabel=$X_3$,
                % zmin=0,
                % zmax=3,
                % xmin=0,
                % xmax=3,
                % ymin=0,
                % ymax=3,
                domain=0:4,
                ticks=none,
                %view={240}{20},
                 axis lines=center,
                 view={110}{25},
                %view={60}{60},
                %unbounded coords=jump,
                %z filter/.expression={z>1 ? nan : z},
                %restrict z to domain*=0:1
                ]

%\draw (0,0,0) node[circle,draw,fill=mycolor1,scale=0.25]{O};

\node[circle,fill=black,inner sep=0pt,minimum size=2pt] (o) at (0,0,0) {};
 
 % x axis
\node[circle,color=mycolor1, fill=mycolor1, inner sep=0pt,minimum size=4pt,label=below right:{}] (b1) at (3,3/2,0) {};

\node[circle,color=mycolor2, fill=mycolor2, inner sep=0pt,minimum size=4pt,label=below right:{}] (b2) at (0,3,3/2) {};

\node[circle,color=mycolor3, fill=mycolor3, inner sep=0pt,minimum size=4pt,label=below right:{}] (b3) at  (3,0, 3/4) {};

\node[circle,color=black, fill=black, inner sep=0pt,minimum size=4pt,label=below right:{}] (b0) at  (3,3/2, 3/4) {};

\draw[very thick,dashed,draw=mycolor1] (o) -- (b1);
\draw[very thick,dashed,draw=mycolor2] (o) -- (b2);
\draw[very thick,dashed,draw=mycolor3] (o) -- (b3);
\draw[very thick,dashed,draw=black] (o) -- (b0);

%\draw[thick,dashed,draw=black] (o) -- (c);

% \node[circle,draw,fill=mycolor1,scale=0.25] (o) at (0,0,0){}; 
% \node[circle,draw,fill=mycolor1,scale=0.25] (b1) at (0,2.5,2.5){};
% \node[circle,draw,fill=mycolor1,scale=0.25] (b2) at (2.5,0,2.5){};
% \node[circle,draw,fill=mycolor1,scale=0.25] (b3) at (2.5,1.25,0){};
% \node[circle,draw,fill=mycolor1,scale=0.25] (c) at (2.5,2.5,2.5){};


% \fill[mycolor1,opacity=0.1] (0,2,2) -- (2.5,2,2) -- (2.5,0,0) --  (0,0,0) --  cycle;
% \fill[mycolor2,opacity=0.1] (2,-2,2) -- (0,-2,0) -- (0,2,0) --  (2,2,2) --  cycle;
% \fill[mycolor3,opacity=0.1] (2.5,1.25,0) -- (0,0,0) -- (0,0,2) --  (2.5,1.25,2) --  cycle;

% \addplot3 [patch, fill=mycolor1!10,draw=none] coordinates {  (0,0,0) (2,0,0) (2,2,2) (0,2,2)
% };

% \addplot3 [patch, fill=mycolor2!10,draw=none] coordinates { (2,0,2) (0,0,0)  (0,2,0)   (2,2,2) 
% };

% \addplot3 [fill=mycolor3!10,draw=none] coordinates { (2.5,1.25,0) (0,0,0)  (0,0,2)   (2.5,1.25,2)
% };
%

 %\closedcycle;
% \addplot3 [fill=red!10,draw=none] coordinates {(0,0,5)(5,0,5)} \closedcycle;

% \addplot3[variable=t, mesh, draw=black!50, domain=-1:1] ({t^2},{t},1);

% \addplot3[surf, opacity=0.35] ({x},{x/2},{0});
% \addplot3[surf, opacity=0.35] (0,{x/2},{x});
% \addplot3[surf, opacity=0.35] {x};
% \addplot3+[mark=none,thick]({0},{y},{0});
% \addplot3[mesh, opacity=0.1, mycolor1, shader=flat,] 
% %coordinates { (2,0,2) (0,0,0)  (0,2,0)   (2,2,2) 
% % };
% %{({x},{x/2},0)};
% ({0},
% {x/2},
% {x});

\addplot3[surf, mycolor1, opacity=0.15, samples=10, shader=flat] ({x},{x/2},{y});

%\addplot3[surf, mycolor3, opacity=0.15, samples=10, shader=flat] ({x},{y},{x/4});

\addplot3[surf, mycolor2, opacity=0.15, samples=10, shader=flat] ({y},{x},{x/2});

\end{axis}
\end{tikzpicture}

==> tikz/histogram.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{brown}{RGB}{165,42,42}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{paleturquoise}{RGB}{175,238,238}
\definecolor{violet}{RGB}{238,130,238}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Normalized Singularity Dimensions },
xmin=-0.039, xmax=1.039,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Density of dimensions},
ymin=0, ymax=5.67753689897313,
ytick style={color=black}
]
\draw[draw=black,fill=paleturquoise,opacity=0.3] (axis cs:0.340327017994275,0) rectangle (axis cs:0.9085381267712,1.75990927412965);
\addlegendimage{ybar,ybar legend,draw=black,fill=paleturquoise,opacity=0.3}
\addlegendentry{80% Confidence Bound for $n=12$}

\draw[draw=black,fill=violet,opacity=0.3] (axis cs:0.427076011175366,0) rectangle (axis cs:0.795005216492022,2.71791416813285);
\addlegendimage{ybar,ybar legend,draw=black,fill=violet,opacity=0.3}
\addlegendentry{80% Confidence Bound for $n=32$}

\draw[draw=black,fill=brown,opacity=0.3] (axis cs:0.472385336285866,0) rectangle (axis cs:0.739861681709806,3.73864835940926);
\addlegendimage{ybar,ybar legend,draw=black,fill=brown,opacity=0.3}
\addlegendentry{80% Confidence Bound for $n=62$}

\draw[draw=none,fill=paleturquoise] (axis cs:0.00999999999999999,0) rectangle (axis cs:0.0366666666666667,0);
\addlegendimage{ybar,ybar legend,draw=none,fill=paleturquoise}
\addlegendentry{n=12}

\draw[draw=none,fill=paleturquoise] (axis cs:0.11,0) rectangle (axis cs:0.136666666666667,0);
\draw[draw=none,fill=paleturquoise] (axis cs:0.21,0) rectangle (axis cs:0.236666666666667,0.00329089829952167);
\draw[draw=none,fill=paleturquoise] (axis cs:0.31,0) rectangle (axis cs:0.336666666666667,0.0271499109710538);
\draw[draw=none,fill=paleturquoise] (axis cs:0.41,0) rectangle (axis cs:0.436666666666667,0.135749554855269);
\draw[draw=none,fill=paleturquoise] (axis cs:0.51,0) rectangle (axis cs:0.536666666666667,1.55772614196421);
\draw[draw=none,fill=paleturquoise] (axis cs:0.61,0) rectangle (axis cs:0.636666666666667,1.92424994007344);
\draw[draw=none,fill=paleturquoise] (axis cs:0.71,0) rectangle (axis cs:0.736666666666667,2.47403563723728);
\draw[draw=none,fill=paleturquoise] (axis cs:0.81,0) rectangle (axis cs:0.836666666666667,2.31940840990995);
\draw[draw=none,fill=paleturquoise] (axis cs:0.91,0) rectangle (axis cs:0.936666666666667,1.55838950668929);
\draw[draw=none,fill=violet] (axis cs:0.0366666666666667,0) rectangle (axis cs:0.0633333333333333,8.85460824262447e-11);
\addlegendimage{ybar,ybar legend,draw=none,fill=violet}
\addlegendentry{n=32}

\draw[draw=none,fill=violet] (axis cs:0.136666666666667,0) rectangle (axis cs:0.163333333333333,3.68763995589474e-07);
\draw[draw=none,fill=violet] (axis cs:0.236666666666667,0) rectangle (axis cs:0.263333333333333,0.000127949268965153);
\draw[draw=none,fill=violet] (axis cs:0.336666666666667,0) rectangle (axis cs:0.363333333333333,0.00934892313536575);
\draw[draw=none,fill=violet] (axis cs:0.436666666666667,0) rectangle (axis cs:0.463333333333333,0.199342643069134);
\draw[draw=none,fill=violet] (axis cs:0.536666666666667,0) rectangle (axis cs:0.563333333333333,2.46739412419151);
\draw[draw=none,fill=violet] (axis cs:0.636666666666667,0) rectangle (axis cs:0.663333333333333,4.09086763665561);
\draw[draw=none,fill=violet] (axis cs:0.736666666666667,0) rectangle (axis cs:0.763333333333333,2.65825148135252);
\draw[draw=none,fill=violet] (axis cs:0.836666666666667,0) rectangle (axis cs:0.863333333333333,0.546738206097449);
\draw[draw=none,fill=violet] (axis cs:0.936666666666667,0) rectangle (axis cs:0.963333333333333,0.0279286673769142);
\draw[draw=none,fill=brown] (axis cs:0.0633333333333333,0) rectangle (axis cs:0.09,6.28688806645066e-18);
\addlegendimage{ybar,ybar legend,draw=none,fill=brown}
\addlegendentry{n=62}

\draw[draw=none,fill=brown] (axis cs:0.163333333333333,0) rectangle (axis cs:0.19,1.50485075826079e-11);
\draw[draw=none,fill=brown] (axis cs:0.263333333333333,0) rectangle (axis cs:0.29,4.90686985952763e-07);
\draw[draw=none,fill=brown] (axis cs:0.363333333333333,0) rectangle (axis cs:0.39,0.000834008921574049);
\draw[draw=none,fill=brown] (axis cs:0.463333333333333,0) rectangle (axis cs:0.49,0.126873837069594);
\draw[draw=none,fill=brown] (axis cs:0.563333333333333,0) rectangle (axis cs:0.59,3.1458481432568);
\draw[draw=none,fill=brown] (axis cs:0.663333333333333,0) rectangle (axis cs:0.69,5.40717799902203);
\draw[draw=none,fill=brown] (axis cs:0.763333333333333,0) rectangle (axis cs:0.79,1.28981509054716);
\draw[draw=none,fill=brown] (axis cs:0.863333333333333,0) rectangle (axis cs:0.89,0.0294210336618712);
\draw[draw=none,fill=brown] (axis cs:0.963333333333333,0) rectangle (axis cs:0.99,2.93968189345407e-05);
\end{axis}

\end{tikzpicture}


==> v6/histogram.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{brown}{RGB}{165,42,42}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{paleturquoise}{RGB}{175,238,238}
\definecolor{violet}{RGB}{238,130,238}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Normalized Singularity Dimensions },
xmin=-0.039, xmax=1.039,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Density of dimensions},
ymin=0, ymax=5.67753689897313,
ytick style={color=black}
]
\draw[draw=black,fill=paleturquoise,opacity=0.3] (axis cs:0.340327017994275,0) rectangle (axis cs:0.9085381267712,1.75990927412965);
\addlegendimage{ybar,ybar legend,draw=black,fill=paleturquoise,opacity=0.3}
\addlegendentry{80% Confidence Bound for $n=12$}

\draw[draw=black,fill=violet,opacity=0.3] (axis cs:0.427076011175366,0) rectangle (axis cs:0.795005216492022,2.71791416813285);
\addlegendimage{ybar,ybar legend,draw=black,fill=violet,opacity=0.3}
\addlegendentry{80% Confidence Bound for $n=32$}

\draw[draw=black,fill=brown,opacity=0.3] (axis cs:0.472385336285866,0) rectangle (axis cs:0.739861681709806,3.73864835940926);
\addlegendimage{ybar,ybar legend,draw=black,fill=brown,opacity=0.3}
\addlegendentry{80% Confidence Bound for $n=62$}

\draw[draw=none,fill=paleturquoise] (axis cs:0.00999999999999999,0) rectangle (axis cs:0.0366666666666667,0);
\addlegendimage{ybar,ybar legend,draw=none,fill=paleturquoise}
\addlegendentry{n=12}

\draw[draw=none,fill=paleturquoise] (axis cs:0.11,0) rectangle (axis cs:0.136666666666667,0);
\draw[draw=none,fill=paleturquoise] (axis cs:0.21,0) rectangle (axis cs:0.236666666666667,0.00329089829952167);
\draw[draw=none,fill=paleturquoise] (axis cs:0.31,0) rectangle (axis cs:0.336666666666667,0.0271499109710538);
\draw[draw=none,fill=paleturquoise] (axis cs:0.41,0) rectangle (axis cs:0.436666666666667,0.135749554855269);
\draw[draw=none,fill=paleturquoise] (axis cs:0.51,0) rectangle (axis cs:0.536666666666667,1.55772614196421);
\draw[draw=none,fill=paleturquoise] (axis cs:0.61,0) rectangle (axis cs:0.636666666666667,1.92424994007344);
\draw[draw=none,fill=paleturquoise] (axis cs:0.71,0) rectangle (axis cs:0.736666666666667,2.47403563723728);
\draw[draw=none,fill=paleturquoise] (axis cs:0.81,0) rectangle (axis cs:0.836666666666667,2.31940840990995);
\draw[draw=none,fill=paleturquoise] (axis cs:0.91,0) rectangle (axis cs:0.936666666666667,1.55838950668929);
\draw[draw=none,fill=violet] (axis cs:0.0366666666666667,0) rectangle (axis cs:0.0633333333333333,8.85460824262447e-11);
\addlegendimage{ybar,ybar legend,draw=none,fill=violet}
\addlegendentry{n=32}

\draw[draw=none,fill=violet] (axis cs:0.136666666666667,0) rectangle (axis cs:0.163333333333333,3.68763995589474e-07);
\draw[draw=none,fill=violet] (axis cs:0.236666666666667,0) rectangle (axis cs:0.263333333333333,0.000127949268965153);
\draw[draw=none,fill=violet] (axis cs:0.336666666666667,0) rectangle (axis cs:0.363333333333333,0.00934892313536575);
\draw[draw=none,fill=violet] (axis cs:0.436666666666667,0) rectangle (axis cs:0.463333333333333,0.199342643069134);
\draw[draw=none,fill=violet] (axis cs:0.536666666666667,0) rectangle (axis cs:0.563333333333333,2.46739412419151);
\draw[draw=none,fill=violet] (axis cs:0.636666666666667,0) rectangle (axis cs:0.663333333333333,4.09086763665561);
\draw[draw=none,fill=violet] (axis cs:0.736666666666667,0) rectangle (axis cs:0.763333333333333,2.65825148135252);
\draw[draw=none,fill=violet] (axis cs:0.836666666666667,0) rectangle (axis cs:0.863333333333333,0.546738206097449);
\draw[draw=none,fill=violet] (axis cs:0.936666666666667,0) rectangle (axis cs:0.963333333333333,0.0279286673769142);
\draw[draw=none,fill=brown] (axis cs:0.0633333333333333,0) rectangle (axis cs:0.09,6.28688806645066e-18);
\addlegendimage{ybar,ybar legend,draw=none,fill=brown}
\addlegendentry{n=62}

\draw[draw=none,fill=brown] (axis cs:0.163333333333333,0) rectangle (axis cs:0.19,1.50485075826079e-11);
\draw[draw=none,fill=brown] (axis cs:0.263333333333333,0) rectangle (axis cs:0.29,4.90686985952763e-07);
\draw[draw=none,fill=brown] (axis cs:0.363333333333333,0) rectangle (axis cs:0.39,0.000834008921574049);
\draw[draw=none,fill=brown] (axis cs:0.463333333333333,0) rectangle (axis cs:0.49,0.126873837069594);
\draw[draw=none,fill=brown] (axis cs:0.563333333333333,0) rectangle (axis cs:0.59,3.1458481432568);
\draw[draw=none,fill=brown] (axis cs:0.663333333333333,0) rectangle (axis cs:0.69,5.40717799902203);
\draw[draw=none,fill=brown] (axis cs:0.763333333333333,0) rectangle (axis cs:0.79,1.28981509054716);
\draw[draw=none,fill=brown] (axis cs:0.863333333333333,0) rectangle (axis cs:0.89,0.0294210336618712);
\draw[draw=none,fill=brown] (axis cs:0.963333333333333,0) rectangle (axis cs:0.99,2.93968189345407e-05);
\end{axis}

\end{tikzpicture}

